DPDist : Comparing Point Clouds Using Deep Point Cloud Distance

We introduce a new deep learning method for point cloud comparison. Our approach, named Deep Point Cloud Distance (DPDist), measures the distance between the points in one cloud and the estimated surface from which the other point cloud is sampled. The surface is estimated locally and efficiently using the 3D modified Fisher vector representation. The local representation reduces the complexity of the surface, enabling efficient and effective learning, which generalizes well between object categories. We test the proposed distance in challenging tasks, such as similar object comparison and registration, and show that it provides significant improvements over commonly used distances such as Chamfer distance, Earth mover's distance, and others.

==> draft.tex <==

%128 figure:
% \begin{figure*}
% \centering
% \begin{subfigure}{.32\textwidth}
%     \centering
% \includegraphics[width=0.98\linewidth]{fig_move_test3Nexp_rand2airplane128.pdf}
% % \caption{Airplane}
%     \label{fig:}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%     \centering
% \includegraphics[width=0.98\linewidth]{fig_move_test3Nexp_rand2car128.pdf}
% % \caption{Car}
%     \label{fig:}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%     \centering
% \includegraphics[width=0.98\linewidth]{fig_move_test3Nexp_rand2table128.pdf}
% % \caption{Table}
%     \label{fig:}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%     \centering
% \includegraphics[width=0.98\linewidth]{fig_rotate_test3Nexp_rand2airplane128.pdf}
% \caption{Airplane}
%     \label{fig:}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%     \centering
% \includegraphics[width=0.98\linewidth]{fig_rotate_test3Nexp_rand2car128.pdf}
% \caption{Car}
%     \label{fig:}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%     \centering
% \includegraphics[width=0.98\linewidth]{fig_rotate_test3Nexp_rand2table128.pdf}
% \caption{Table}
%     \label{fig:}
% \end{subfigure}
% \caption{Translation (top) and rotations (bottom) detection experiments evaluate on (a) "Airplane" (b) "Car", and (c) "Table" as before. Remarkably, DPDist is still the best method, although the SPD was  trained over another category ("Chair'") and not over these categories. The generalization ability is a result of using local surface modelling.   }
% \label{fig:results:local_presentation_rubastness}
% \end{figure*}








%intro:
% ; thus, it is unnatural input of a neural network. 
% Neural networks have already proven their benefits in many 2D  vision tasks. Recent methods tackled the challenge of applying neural networks on 3D point clouds and show promising results on various 3D vision tasks e.g.  classification, segmentation,  \cite{qi2017pointnet,qi2017pointnet++,zaheer2017deep,ben20183dmfv}
% % ,dgcnn,voxnet, and many more}
% , auto-encoders \cite{yang2018foldingnet,groueix2018atlasnet}
% % ,more}
% , GANs\cite{achlioptas2017learning}, registration \cite{wang2019deep,aoki2019pointnetlk,sarode2019pcrnet}.
% % , image to 3D reconstruction\cite{}, normal estimation\cite{}, . % normal estimation too maybe? and cite nesti-net and pcpnet? your call

% Many tasks (e.g classification) result in a categorical output which is optimized using a loss function that compares the output to ground truth labels directly. However, in other tasks like registration, the output is a transformation between two input point clouds A and B. While it is generally possible to regress the transformation parameters, it is common practice to compare between the transformed point cloud A and the ground truth point cloud B. Currently, the most commonly used loss functions for comparing between 3D point clouds are Chamfer Distance (CD) and Earth Mover's Distance (EMD).

% In this paper, we introduce a deep learning framework to compare between two point cloud representation of surfaces directly from the raw points. 
% We use a neural network to estimate the distance of each point from a local surface in the other point cloud. Then we combine it to a bi-directional distance metric.

%registration:
% The results show that for point cloud inputs with fewer than 1024 points, PCRNet outputs an unstable parameters output. %IBS do we have a result supporting that? if not consider removing this or canging the start to "when experimenting with PCRNET we witnessed... 
% When performing its iterative version (for more details please see \cite{sarode2019pcrnet}), we noticed that the error is spiking from $~0$ to 180 degrees and back. We solved this problem by limiting the output rotation angle to maximum of 45 degrees. We results with iterative PCRNet decreasing monotonically between iterations, like the original version of PCRNet. This stabled version is suitable to evaluate it performance over less than 1024 points.
%IBS: I know that this is something that you did but im not sure it is important to the paper. it basically trashes the PCRNet guys work, we dont want to do that, they may be our reviewers... 
% Due to inherent training stability issues in PCRNet, we limit the output rotation angle to maximum of 45 degrees to yield a monotonically decreasing training curve for point clouds with fewer than 1024 points. 
% The procedure is done by referring to the four rotation parameters as an angle and three parameters for direction, instead of four unit quaternions directly (both options are quaternions versions). %IBS: not sure about this line, maybe cite a book where these two options appear? 

%training SPD:

% For training the SPD network, we need to sample points and calculate their true distance from a CAD surface. 
% We first normalize the CAD models to fit within the unit sphere. Then, For each CAD model we sample 10k points in the following sampling protocols (total of 30k points per CAD model):
% \begin{enumerate}
%     \item Uniform sampling on the surface, using FPS \cite{eldar1997farthest}. 
%     \item Random sampling within maximum distance of 0.1 from the surface ($5\%$ of bounding box $[-1,1]$).
%     \item Random sampling in the unit cube.
% \end{enumerate}
% Note that Each sampled point's true distance from the surface is stored as ground truth distance.
 
% % We can train DPDist for a specific category and specific number of input points $T$. Further details are provided in the supplementary.

% The training procedure is as follow:
% For each CAD model we sample two sets of points $S_A$ and $S_B$, where $S_A$ represent the surface $A$, and $S_B$ is a set of query points which we want to learn their distance from surface $A$.
% $S_A$ is a set of $N$ points sampled on the surface (protocol 1). $S_B$ is a set of $N$ points, composed of the three sampling protocols above where $0.5N$ are are sampled using protocol 1 (on the surface), $0.25N$ using protocol 2 (with distance smaller than 0.1), and $0.25N$ using protocol 3 (anywhere in the unit cube).

% % The second set is our Ground Truth (GT). 
% We feed $S_A$ to our surface representation network, and each query point in $S_B$ to our localization procedure.
% SPD learns the distance between each point from $S_B$ to $A$.


% For each point in $S_B$ we extract a local representation of $A$, thus, SPD learns distances from multiple local patches for each CAD model, i.e. using a batch size of 16, and $128$ points yields $2048$ local patches in each optimization step.


%rotation test figure:
% \begin{figure*}
% \centering
% \begin{subfigure}{.32\textwidth}
%     \centering
% \includegraphics[width=0.98\linewidth]{fig_rotate_testchair64.pdf}
% \caption{}
%     \label{fig:fig_rotate_testchair64}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%     % \centering
%     \includegraphics[width=0.98\linewidth]{fig_rotate_testchair128.pdf}
%     \caption{}
%     \label{fig:fig_rotate_testchair128}
% \end{subfigure}
% \begin{subfigure}{.32\textwidth}
%     % \centering
%     \includegraphics[width=0.98\linewidth]{fig_rotate_testchair256.pdf}
%     \caption{}
%     \label{fig:fig_rotate_testchair256}
% \end{subfigure}
% \caption{Rotation test -  We evaluate DPDist and the other methods for sampling robustness by testing its ability identify a new sample as closer than a rotated version of itself with different rotation magnitudes.}
% \label{fig:rotate}
% \end{figure*}

%RW
% \subsection{3D shape descriptors}
% Before the age of deep learning, hand crafted features were a popular choice for many shape analysis tasks, including object recognition, matching, retrieval, and registration. These descriptors are commonly based on low-level geometry e.g. Euclidean distance, normal vectors, or principal curvatures. They can be divided into two groups: local descriptors \cite{FPFH, SI, SHOT}, and global descriptors \cite{OUR-CVFH, ESF, GRSD}. A recent comprehensive performance analysis \cite{Gou} suggests guidelines for descriptor selection per task, it remain non-trivial and highly data dependent. Therefore, these descriptors are not good candidates for comparing between point clouds. 
%IBS I think this paragraph can be removed if there is a length issue. The hand crafted descriptors seem to be orthogonal to our narrative (they were not used in the direct context of comparing point clouds and we are not using them in the baseline comparisons). 

% The point cloud is sampled using farthest point sampling (FPS) \cite{eldar1997farthest} and local features are extracted from each sampled point and its neighbors. The points are then grouped and PointNet is applied again to the next level in the hierarchy. This method is able to represent local geometry in the expense of computation time and complexity since it requires extracting each point's neighborhood and computing a local and regional PointNet features. Every local neighborhood is computed separately, thus, each point contributes to many local representations, yet its PointNet representation is needed to recompute separately with respects to the specific local neighborhood origin.

% Here, the grid provides the structure and the modified Fisher Vector the order invariant and number of points' independence. 
% 3DmFV achieved  better results than the basic PointNet; thus, it is a favorable global representation.

%PCRNet
 
% first it maps both the source and the target point clouds into two PointNet global embedding vectors   \cite{qi2017pointnet}.  Then, it feeds both vectors into a pose estimation network, that provides the transformation parameters.  
% translation parameters and quaternion rotation parameters.
% Using these parameters a transformation is performed on the source and and then the distance between the transformed source and the target is measured. 
% The distance  measure that is used is  is used as the neural network's loss function; thus, choosing Chamfer distance or EMD highly affects the network's performance.

%traiing data
% The motivation for this sampling procedure is to train over half points from the surface and half off-surface points.
% uniformly using FPS from the surface and shuffled; then, we use the first $N$ shuffled points as the point cloud that describes the surface, and from the other $N$ points we take $\frac{N}{2}$ as query points.
% We added an additional set of $\frac{N}{2}$ query points, where $\frac{N}{4}$ points are within a distance of 0.1 from the surface, and $\frac{N}{4}$ points are located randomly in the unit cube.
% We limit the distance to 0.1 because it aids in learning small geometric details (as seen in DeepSDF \cite{park2019deepsdf}) This results in $N$ points that represent the CAD model and $N$ query points.
